On the Nystrom Approximation for Preconditioning in Kernel Machines

Kernel methods are a popular class of nonlinear predictive models in machine learning. Scalable algorithms for learning kernel models need to be iterative in nature, but convergence can be slow due to poor conditioning. Spectral preconditioning is an important tool to speed-up the convergence of such iterative algorithms for training kernel models. However computing and storing a spectral preconditioner can be expensive which can lead to large computational and storage overheads, precluding the application of kernel methods to problems with large datasets. A Nystrom approximation of the spectral preconditioner is often cheaper to compute and store, and has demonstrated success in practical applications. In this paper we analyze the trade-offs of using such an approximated preconditioner. Specifically, we show that a sample of logarithmic size (as a function of the size of the dataset) enables the Nystrom-based approximated preconditioner to accelerate gradient descent nearly as well as the exact preconditioner, while also reducing the computational and storage overheads.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Not applicable] 
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL).  [Not applicable] \\
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> sections/hs_norm.tex <==
\mysection{Auxiliary Lemmas}\label{sec:HS_norm_bound}
\pp{Perhaps this section title should be ``Proof of \Cref{proposition:HSbound}'', and we start by rewriting the proposition statement verbatim and then go on to prove it with intermediate lemmas.}
We start by stating a more general version of the result in \Cref{proposition:HSbound_special}.
\begin{proposition}\label{proposition:HSbound}
Suppose $\mcK, \mcK' \in L(\Hilbert)$ are finite rank, self-adjoint positive semidefinite operators with eigenvalues $\lambda_1 \geq \lambda_2 \geq \dotsc$ and $\lambda_1' \geq \lambda_2' \geq \dotsc$, respectively. 
Assume that $q$ is such that $\lambda_{q}, \lambda_{q}' > 0$.
%Then $\norm{\mathcal{P} - \mathcal{P}'}_{HS} \leq xxx$.
Define $\mcP, \mcP' \in L(\Hilbert)$ given by $\mcP = \lambda_{q} f_{\lambda_{q}}(\mcK)^{-1}$ and $\mcP' = \lambda_{q}' f_{\lambda_{q}'}(\mcK')^{-1}$.
Then
\[
(\forall f\neq 0) \quad \frac{\norm{\mcP f}}{\norm{\mcP' f}} \in [(1+\eps')^{-1},1+\eps']
\]
where $\eps' 
= \frac{1}{\lambda_{q}}\hsnorm{ \mcK - \mcK'} + \abs{\frac{1}{\lambda_{q}}-\frac{1}{\lambda_{q'}}}\hsnorm{\mcK' } 
% \leq \frac{\hsnorm{\mathcal{K} - \mathcal{K}'}}{\lambda_{q}}\left(1 + \frac{\hsnorm{\mcK'}}{\lambda_{q}'}\right)
$.
\end{proposition}

% \begin{proposition}\label{prop:beta_bound}
% $\hsnorm{\mcK},\hsnorm{\mcK'} \leq \beta(K)$ and $\hsnorm{\mcK^{\frac12}},\hsnorm{\mcK'^{\frac12}} \leq \sqrt{\beta(K)}$ .
% \end{proposition}
% \begin{proof}
% Observe that we have,
% \begin{align*}
%  &\hsnorm{\mcK}\leq \norm{\mcK}_* = \frac1n \sum_{i=1}^n K(x_i,x_i) \leq \underset{i}{max}\: K(x_i,x_i) \leq \underset{x}{max}\: K(x,x) =\beta(K)\\
%  &\hsnorm{\mcK^{\frac12}}= \sum_{i=1}^n \lambda_i(\mcK)
% \end{align*}
% Where$\norm{}_*$ is the trace norm. Similar reasoning for $\hsnorm{\mcK'}$ and $\hsnorm{\mcK'^{\frac12}}$.

% \hsnorm{\mcK} &= \hsnorm{\frac1n \sum_{i=1}^n K(\x_i,\cdot)\otimes K(\x_i,\cdot)} \leq \underset{i}{\rm max}\hsnorm{K(\x_i,\cdot) \otimes K(\x_i,\cdot)}\\
% &= \underset{i}{\rm max}\: \norm{K(\x_i,\cdot)}_{\Hilbert}^2 = \underset{i}{\rm max}\: K(\x_i, \x_i)\leq\underset{x}{\rm max}\: K(\x, \x) = \beta(K)
% where we have used the fact that for a rank-1 operator $f\otimes f$ the Hilbert-Schmidt norm equals $\norm{f}^2$. Similar proof can be repeated for $\mcK'$.

% \details{alternative proof: HS $\leq$ trace norm $=1/n$ sum diag $\leq$ max diag?}
% \end{proof}



% In this section, we show that when two finite rank operators $\mcK$ and $\mcK'$ are close in the \HS\ norm, their corresponding preconditioners are similarly close \emph{in a multiplicative sense}.
% The results in this section do not use properties of RKHS and hold for any separable Hilbert space $\Hilbert$.
% %To lay the groundwork for this, we first delineate two auxiliary lemmas, which subsequently inform the primary proposition concluding this section.\lnote{xxx}

% The first step, \cref{lemma:rationbound}, states that all we need is to find an upper bound for $\opnorm{\mathcal{P}-\mathcal{P}'}$ and a lower bound for the eigenvalues of $\mathcal{P}$ and $\mathcal{P}'$. 
% In \cref{sec:operator} we discuss potential alternatives to directly bound the operator norm, however, in the rest of the section we find a bound for $\hsnorm{\mathcal{P}-\mathcal{P}'}$ and since this is an upper bound for $\opnorm{\mathcal{P}-\mathcal{P}'}$ we can apply lemma \ref{lemma:rationbound}.%\lnote{update depending on whether we keep op norm section, probably move to intro to justify the op norm section}
\iffalse
\begin{lemma}%\label{lemma:rationbound}
Let $\mathcal{P}$ and $\mathcal{P}'$ be two operators in $\Hilbert$, where $\lambda_{min}(\mathcal{P})$ and $\lambda_{min}(\mathcal{P}')$ denote their smallest eigenvalues, respectively.\lnote{need to cite spectral theorem here. how do you define and ensure existence of eigenvalues? what are the assumptions on P? are they bounded operators?} 
Assume that $\lambda_{min}(\mathcal{P}), \lambda_{min}(\mathcal{P}') \geq \lambdamin$. 
Additionally, suppose the spectral norm of their difference is bounded $\epsilon>0$, i.e., $\norm{\mathcal{P}-\mathcal{P}'}_{OP} \leq \epsilon$. Under these conditions, we can establish a lower bound $\forall f\in\Hilbert\: s.t.\: \norm{f}_{\Hilbert}=1$\lnote{enought to exclude 0} on the relative ratio as follows:
\[
\frac{1}{1+\frac{\epsilon}{\lambdamin}}
\leq \frac{\norm{\mathcal{P}(f)}}{\norm{\mathcal{P}'(f)}} 
\leq 1+\frac{\epsilon}{\lambdamin}
\]
\end{lemma}

\begin{proof}
\begin{align*}
&\frac{\norm{\mathcal{P}(f)}}{\norm{\mathcal{P}'(f)}} = \frac{\norm{\mathcal{P}(f)}}{\norm{(\mathcal{P}'-\mathcal{P})(f)+\mathcal{P}(f)}}\geq \frac{\norm{\mathcal{P}(f)}}{\epsilon+\norm{\mathcal{P}(f)}} = \frac{1}{\frac{\epsilon}{\norm{\mathcal{P}(f)}_2}+1}\geq \frac{1}{1+\frac{\epsilon}{\lambdamin}} \approx 1-\frac{\epsilon}{\lambdamin} \\
&\frac{\norm{\mathcal{P}(f)}}{\norm{\mathcal{P}'(f)}} = \frac{\norm{(\mathcal{P}-\mathcal{P}')(f)+\mathcal{P}'(f)}_2}{\norm{\mathcal{P}'(f)}}\leq \frac{\epsilon+\norm{\mathcal{P}'(f)}}{\norm{\mathcal{P}'(f)}}=\frac{\epsilon}{\norm{\mathcal{P}'(f)}}+1\leq 1+\frac{\epsilon}{\lambdamin} %\qedhere
\end{align*}
\end{proof}
\fi
% \begin{lemma}\label{lemma:rationbound}
% Let $\mathcal{A}, \mathcal{B} \in L(\Hilbert)$ be such that for all $f \in \Hilbert$, $\norm{\mcA f} \geq \lambdamin \norm{f}$ and $\norm{\mcB f} \geq \lambdamin \norm{f}$. 
% Additionally, assume $\opnorm{\mathcal{A}-\mathcal{B}} \leq \epsilon$. 
% Then for all $f \in \Hilbert$ we have
% $(1+\frac{\eps}{\lambdamin})^{-1}\norm{\mcB f } \leq \norm{\mcA f} \leq (1+\frac{\eps}{\lambdamin})\norm{\mcB f }$.
% \end{lemma}
% \begin{proof}
% By symmetry it is enough to prove the right hand side inequality:  $\norm{\mcA f} = \norm{\mcA f - \mcB f + \mcB f} \leq \norm{\mcB f} + \eps \norm{x} \leq \norm{\mcB f} (1+\frac{\eps}{\lambdamin})$.
% \end{proof}

% The next step, \cref{lem:equivalences}, is the observation that the quality of the multiplicative approximation in \cref{lemma:rationbound} is invariant under taking inverses of the operators.
% It turns out that it will be easier to bound $\hsnorm{\mathcal{P}^{-1} - \mathcal{P}'^{-1}}$ and apply \cref{lemma:rationbound} to $\mathcal{P}^{-1}$ and $\mathcal{P}'^{-1}$.
% As a bonus, in that case we can take $\lambdamin = 1$.\lnote{was: We introduce the following lemma to eliminate the need for a lower bound for $\lambdamin$ in the previous lemma.}
% \begin{lemma}\label{lem:equivalences}
% Let $\mcA, \mcB \in L(\Hilbert)$ be self-adjoint and invertible\details{implies with bounded inverse for free by the closed graph theorem}.
% Let $c \geq 1$.
% The following statements are equivalent:
% \begin{enumerate}
% \item $(\forall f\neq 0) \frac{\norm{\mcA f}}{\norm{\mcB f}} \in [c^{-1},c]$.
% \item $\opnorm{\mcA\mycirc \mcB^{-1}}, \opnorm{\mcB\mycirc \mcA^{-1}}  \in [c^{-1},c]$.
% \item $\opnorm{\mcB^{-1}\mycirc \mcA}, \opnorm{\mcA^{-1}\mycirc \mcB}  \in [c^{-1},c]$.
% \item $(\forall f\neq 0) \frac{\norm{\mcA^{-1} f}}{\norm{\mcB^{-1} f}} \in [c^{-1},c]$.
% \end{enumerate}
% \end{lemma}
% \begin{proof}
% ($1 \Leftrightarrow 2$) 
% In 1, use substitution $f = \mcB^{-1} (g)$ to get $(\forall g\neq 0) \frac{\norm{\mcA \mycirc\mcB^{-1} (g)}}{\norm{g}} \in [c^{-1},c]$.
% Taking $\sup$ we get $\opnorm{\mcA \mycirc\mcB^{-1}} \in [c^{-1},c]$.
% Similarly, in 1 use substitution $f = \mcA^{-1} g$ and take $\inf$ to get $\opnorm{\mcB^{-1} \mycirc\mcA} \in [c^{-1},c]$.
% The same argument in reverse completes the equivalence.

% ($2 \Leftrightarrow 3$) 
% Follows immediately from the fact that the operator norm is invariant under taking adjoint.

% ($3 \Leftrightarrow 4$)
% This follows from $1 \Leftrightarrow 2$ with $\mcA^{-1}$ in the role of $\mcA$ and $\mcB^{-1}$ in the role of $\mcB$.
% \end{proof}

% The challenge with working directly with $\mcP$ and $\mcP'$ is that their $\lambda_{\lmin}$ values can be arbitrarily small, making them difficult to handle. 
% However, by switching our focus to  $\mcP^{-1}$ and $\mcP'^{-1}$ and find a $c$ such that $\frac{1}{c}\leq\frac{\norm{\mcP^{-1}(f)}}{\norm{\mcP'^{-1}(f)}}\leq c,\:\forall f\in\Hilbert$ then the same $c$ will satisfy $\frac{1}{c}\leq\frac{\norm{\mcP(f)}}{\norm{\mcP'(f)}}\leq c,\:\forall f\in\Hilbert$ because of lemma $\ref{lem:equivalences}$. Now the $\lambda_{min}$ for both $\mcP^{-1}$ and $\mcP'^{-1}$ is $1$, and we can focus to just bound $\hsnorm{\mcP^{-1}-\mcP'^{-1}}$.

In the next proposition, the main result of the section, we bound $\hsnorm{\mathcal{P}^{-1} - \mathcal{P}'^{-1}}$ and apply the previous two lemmas.
%\details{Note that in our case $\hsnorm{\mcK} \leq \kappa$: by triangle inequality $\hsnorm{\mcK} = \hsnorm{\frac{1}{n}\sum_i k_{x_i} \otimes k_{x_i}} \leq \lmax_i \hsnorm{k_{x_i} \otimes k_{x_i}} = \lmax_i \hnorm{k_{x_i}}^2 = \lmax_i K(x_i, x_i) \leq \kappa$ (recall $k_{x} \otimes k_{x}:\mcH \to \mcH, f \mapsto f(x) k_{x} $). \anote{I added the proof of this in main Theorem \ref{theorem:main}.
%}}
% \begin{proof}(of \Cref{proposition:})
% %For an operator $\mcA \in L(H)$, let $T(\mcA):= \mcA + \proj_{\nullspace(\mcA)^\perp}$, $T(\mcA) \in L(H)$ denote the ``extension'' of $\mcA$ as identity on its nullspace. 
% %
% %We can write $\mcP^{-1} = T(\frac{1}{\lambda_{q}} f_{\lambda_{q}}(\mcK))$ and similarly for $\mcP'$. 
% %We can write $\mcP^{-1} = \frac{1}{\lambda_{q}} f_{\lambda_{q}}(\mcK)$ and similarly for $\mcP'$. 
% %\lnote{xxx}
% %We have $ \hsnorm{\mcP - \mcP'} \leq xxx $.
% %
% \details{Old, part of alternate bound: Let $\eps = \hsnorm{\mathcal{K} - \mathcal{K}'}$.}
% Let $V = \image(\mcK) + \image(\mcK')$. 
% Below, if $\mcA \in L(\Hilbert)$ is such that $\mcA|_V$ has image in $V$, then (by a slight abuse of notation) we consider $\mcA|_V$ as an element of $L(V)$ (even though in general $\mcA|_V:V \to \Hilbert$).
% We also use notation $\HS(\Hilbert)$ and $\HS(V)$ to denote the Hilbert-Schmidt norm for operators on $\Hilbert$ and $V$, respectively.
% We have 
% \begin{align*}
% \hsnorm[(\Hilbert)]{\mcP^{-1} - \mcP'^{-1}} 
% &= \hsnorm[(\Hilbert)]{\rfrac{1}{\lambda_{q}} f_{\lambda_{q}}(\mcK) - \rfrac{1}{\lambda_{q}'} f_{\lambda_{q}'}(\mcK')} \\
% &= \hsnorm[(V)]{\rfrac{1}{\lambda_{q}} f_{\lambda_{q}}(\mcK|_{V}) - \rfrac{1}{\lambda_{q}'} f_{\lambda_{q}'}(\mcK'|_{V})} \\
% &= \hsnorm[(V)]{\rfrac{1}{\lambda_{q}} f_{0}\bigl((\mcK - \lambda_{q}\mcI)|_{V}\bigr) - \rfrac{1}{\lambda_{q}'} f_{0}\bigl((\mcK' - \lambda_{q}'\mcI)|_{V}\bigr)} \\
% &= \hsnorm[(V)]{ f_{0}\bigl((\rfrac{1}{\lambda_{q}}\mcK - \mcI)|_{V}\bigr) - f_{0}\bigl((\rfrac{1}{\lambda_{q}'} \mcK' - \mcI)|_{V}\bigr)} \\
% &\leq \hsnorm[(\Hilbert)]{ \rfrac{1}{\lambda_{q}}\mcK - \rfrac{1}{\lambda_{q}'} \mcK' } \\
% %
% %&= \hsnorm{ \frac{1}{\lambda_{q}}\mcK - \frac{1}{\lambda_{q}}\mcK' + \frac{1}{\lambda_{q}}\mcK' - \frac{1}{\lambda_{q}'} \mcK' } \\
% &\leq \hsnorm[(\Hilbert)]{ \frac{1}{\lambda_{q}}(\mcK - \mcK')} + \hsnorm[(\Hilbert)]{\frac{\lambda_{q}' - \lambda_{q}}{\lambda_{q}\lambda_{q}'}\mcK' } := \eps' \\
% % &\color{red}= \left|\frac{1}{\lambda_{q}}\right|\cdot\hsnorm{ (\mcK - \mcK')} + \left|\frac{\lambda_{q}' - \lambda_{q}}{\lambda_{q}\lambda_{q}'}\right|\cdot\hsnorm{\mcK' } := \eps'\\
% %&\leq \frac{1}{\lambda_{q}} \hsnorm{ \mcK -  \mcK' } + \frac{\hsnorm{\mathcal{K} - \mathcal{K}'}}{\lambda_{q}\lambda_{q}'} \hsnorm{\mcK'} \\
% &\leq \lambda_{q}^{-1} \hsnorm[(\Hilbert)]{\mathcal{K} - \mathcal{K}'} \left(1 + \lambda_{q}'^{-1}\hsnorm[(\Hilbert)]{\mcK'}\right).
% \end{align*}
% \details{restriction needed because otherwise it is not H-S.}
% \details{alternative, in triangle inequality, can change added and removed term:
% \begin{align*}
% &= \hsnorm{ \frac{1}{\lambda_{q}}\mcK - \frac{1}{\lambda_{q}'}\mcK + \frac{1}{\lambda_{q}'}\mcK - \frac{1}{\lambda_{q}'} \mcK' } \\
% &= \hsnorm{ \frac{\lambda_{q}' - \lambda_{q}}{\lambda_{q}\lambda_{q}'}\mcK + \frac{1}{\lambda_{q}'}(\mcK - \mcK') } \\
% &\leq \frac{\eps}{(\lambda_{q}-\eps)^2} \hsnorm{\mcK} + \frac{1}{\lambda_{q}-\eps} \hsnorm{ \mcK -  \mcK' }\\
% &\leq \frac{\eps}{\lambda_{q}-\eps}(1 + \frac{\hsnorm{\mcK}}{\lambda_{q}-\eps}) := \eps'.
% \end{align*}
% }
% %\lnote{Operator norm bound would be $ O(\log \dim V) \frac{\opnorm{\mathcal{K} - \mathcal{K}'}}{\lambda_{q}}(1 + \frac{\opnorm{\mcK'}}{\lambda_{q}'})$.}
% %We have $\hsnorm{f_{\lambda_{q}}(\mcK) - f_{\lambda_{q}'}(\mcK')} = \hsnorm{f_0()+\lambda}$.

% From \cref{lemma:rationbound} with $\lambdamin=1$ and the fact that $\opnorm{\cdot}\leq\hsnorm{\cdot}$ we get 
% \[
% (\forall f\neq 0) \quad \frac{\norm{\mcP^{-1} f}}{\norm{\mcP'^{-1} f}} \in [(1+\eps')^{-1},1+\eps'].
% \]
% With \cref{lem:equivalences} this implies the claim.
% % With \cref{lem:equivalences} this implies 
% % \[
% % (\forall f\neq 0) \quad \frac{\norm{\mcP f}}{\norm{\mcP' f}} \in [(1+\eps')^{-1},1+\eps'].
% % % \qedhere
% % \]
% \end{proof}


